Inferring Galactic Parameters from Chemical Abundances: A Multi-Star Approach

Constraining parameters such as the initial mass function high-mass slope and the frequency of type Ia supernovae is of critical importance in the ongoing quest to understand galactic physics and create realistic hydrodynamical simulations. In this paper, we demonstrate a method to precisely determine these using individual chemical abundances from a large set of stars, coupled with some estimate of their ages. Inference is performed via the simple chemical evolution model Chempy in a Bayesian framework, marginalizing over each star's specific interstellar medium parameters, including an element-specific `model error' parameter to account for inadequacies in our model. Hamiltonian Monte Carlo (HMC) methods are used to sample the posterior function, made possible by replacing Chempy with a trained neural network at negligible error. The approach is tested using data from both Chempy and the IllustrisTNG simulation, showing sub-percent agreement between inferred and true parameters using data from up to 1600 individual stellar abundances. For IllustrisTNG, strongest constraints are obtained from metal ratios, competitive with those from other methods including star counts. Analysis using a different set of nucleosynthetic yields shows that incorrectly assumed yield models can give non-negligible bias in the derived parameters; this is reduced by our model errors, which further show how well the yield tables match data. We also find a significant bias from analyzing only a small set of stars, as is often done in current analyses. The method can be easily applied to observational data, giving tight bounds on key galactic parameters from chemical abundances alone.

==> advi_old.tex <==


% \subsection{Automatic Differentiation Variational Inference (ADVI)}\label{appen: ADVI}
% For the many-parameter models (for example our analysis with large $n_\mathrm{stars}$), exact MCMC methods become inefficient and we must look to approximate methods to sample the posterior function. Here we use `Automatic Differentiation Variational Inference' \citep[ADVI; ][]{2013arXiv1312.6114K,2016arXiv160300788K,2017arXiv170309194R}, which approximates the posterior function as a product of univariate Gaussians, which we can trivially sampled from. The posterior approximation depends on a number of latent parameters (describing the means and standard deviations of each Gaussian), and optimizations are performed via gradient-descent, which requires our model to be differentiable. Notably, any bounded variables are transformed to unbounded space before the optimization is performed, which allows application to strictly-positive quantities for example.

% There are three commonly used type of ADVI approximations:
% \begin{enumerate}
%     \item \textbf{Mean Field ADVI}. This is the most basic form of the algorithm with all input variables assumed to be uncorrelated, leading to the posterior being approximated as a spherical Gaussian. This is often a gross oversimplification that may lead to significant biases in computed posterior chain sample statistics.  Previous \textit{Chempy} analyses noted strong correlations between the global $\alpha_\mathrm{IMF}$ and $\log_{10}(N_\mathrm{Ia})$ parameters \citepalias{chempy}, indicating that this is a poor assumption here. 
%     \item \textbf{Full Rank ADVI}. An improvement upon Mean Field ADVI, this accounts for parameter correlations by additionally optimizing a covariance matrix between all parameters. Using $n_\mathrm{par}$ parameters \oliver{check nomenclature for this}, the correlation matrix has $\frac{1}{2}n_\mathrm{par}(n_\mathrm{par}+1)$ non-trivial entries, thus this adds significant computational expense at for a high-dimensional posterior. 
%     \item \textbf{`Group' ADVI}. This is a cross between the two ADVI approaches above, where we allow only a subset of parameters to be correlated. In our context, we allow for correlations between the $(2+n_\mathrm{el})$ global variables $\vec\Lambda$ and $\Sigma$, assuming the $4n_\mathrm{stars}$ local variables $\{\vec\Theta_i,T_i\}$ are uncorrelated. This has lower accuracy than the fully covariant approach, but is faster to compute since the correlation matrix size 
%     is independent of $n_\mathrm{stars}$.
% \end{enumerate}

% The great strength of ADVI is its speed; we can approximately sample very high-dimensional posteriors in a fraction of the CPU-time taken by HMC. For large data-sets we can also apply the `mini-batch' technique, using only a fraction of the stellar data-points to update gradients in each epoch, allowing for lower memory use and faster computation. One drawback, however, is that ADVI cannot be simply parallelized (unlike HMC) due to its iterative algorithm structure. 


%\section{Inference using ADVI}\label{appen: ADVI_results}
%Here we present inference results for the TNG mock data-set using ADVI rather than HMC sampling, which allows us to probe larger values of $n_\mathrm{stars}$. In this analysis, we implement both `Full Rank' and `Group' ADVI in \texttt{PyMC3}, utilizing a maximum of $10^5$ steps to fit the Gaussian posterior approximations to the true posterior. We allow the algorithm to stop prematurely when the loss function (between true and approximate distributions) has stopped decreasing to within $0.1\%$. Since ADVI is an inexact method, it is important to compare the output to full HMC results to ensure the validity of the Gaussian approximations. From the posterior corner plot (Fig.\,\ref{fig: TNG_corner_plot}), it seems that the model error parameters are strongly non-Gaussian here; they may still be adequately fit by ADVI, since all variables are transformed to a continuous non-bounded space (for example by taking a logarithm), which significantly reduces the non-Gaussianity.

%In Fig.\,\ref{fig: TNG_comparison} we show the inferred global parameter median and $1\sigma$ bounds as a function of $n_\mathrm{stars}$ for HMC and the two ADVI methods. Here, we include results only from a single set of stars for each sized data-set, thus we are subject to significant bias from the choice of star for small samples. As previously mentioned, the correlation matrix in Full Rank ADVI scales as $n_\mathrm{stars}^2$, thus this inference is performed only up to $n_\mathrm{stars}=100$, along with the HMC inference. 

%\oliver{note agreements}
%The median parameter inference is shown to be in good agreement between the three models, 

%The variance does this....
% There is seen to be negligible difference between global parameters inferred from HMC and Full Rank ADVI here, showing the validity of the Gaussian approximations. The constraints from Group ADVI are similar again, with no significant change in the parameter variances, unlike that found for mock data. This may be partly explained by the number of extra degrees of freedom added by the model error parameters, which can allow for more flexible fitting of the incorrect spherical Gaussian model. Fig.\,\ref{fig: TNG_comparison_times} also shows similar results to before, with much reduced computation time for Group ADVI in the case of many stars. As before, the computation time for HMC and Full Rank ADVI becomes very large for $n_\mathrm{stars}>200$, thus we only use the Group ADVI algorithm in this regime.

% From Fig.\,\ref{fig: mock_comparison}, we note no significant discrepancies between HMC and Full Rank ADVI sampling (except for a tiny positive shift of the Full Rank ADVI predictions compared with HMC), indicating that approximation of the posterior by a fully covariant Gaussian is valid in this instance. For Group ADVI (where we consider only correlations between global parameters), there is a clear underestimation of both parameters variances for small $n_\mathrm{stars}$ indicating poor fitting, but this is negligible with many stars. This can be rationalized by noting that at low $n_\mathrm{stars}$, there are fewer local parameters and thus fewer degrees of freedom for the fitting of an incomplete Gaussian model, leading to more inaccurate predictions. In Fig.\,\ref{fig: mock_comparison_times}, we note similar sampling times between all methods at low $n_\mathrm{stars}$, but above 200 stars, the convergence timescales become very large for HMC and Full Rank ADVI, but remain manageable for Group ADVI. Unlike other methods, HMC can be run in parallel, thus is quoted run-time (using 16-cores) is significantly smaller than the equivalent single-core speed (by a factor of $19/4$ rather than 16 in this case, due to the necessity of running tuning steps on each core individually). In the limit of high $n_\mathrm{stars}$, Group ADVI becomes the most useful sampling method, and has a similar run-time as HMC for $10\times$ the amount of data. For this reason Group ADVI was the only algorithm used for $n_\mathrm{stars}>200$.

%\oliver{add time details}
%Fig.\,\ref{fig: TNG_times} shows the sampling times for the inference methods shown in Fig.\,\ref{fig: TNG_comparison}.

%\oliver{check these conclusions}.
%From this, we note that the posterior used in this paper (Eq.\,\ref{eq: posteroir}) is found to be well approximated by a Gaussian (at least for the inference of $\vec\Lambda$ sample statistics), affording accurate sampling at low computational cost for high $n_\mathrm{el}$.

% Considering the HMC tracks of figure \ref{fig: mock_comparison} (the most accurate sampling method) we note that the median posterior values of $\alpha_\mathrm{IMF}$ and $\log_{10}(N_\mathrm{Ia})$ approach the true values of $-2.3$ and $-2.89$ as $n_\mathrm{stars}$ becomes large, with all estimates within $1\sigma$ ($2\sigma$) for $\alpha_\mathrm{IMF}$ ($\log_{10}(N_\mathrm{Ia})$).  Indeed, the HMC sampling for $n_\mathrm{stars} = 200$ and the Group ADVI approximations for $n_\mathrm{stars}=1000$ give  $\alpha_\mathrm{IMF}$ ($\log_{10}(N_\mathrm{Ia})$) bounds of $-2.302\pm0.005$ and  $-2.299\pm0.001$ ($-2.880\pm0.006$ and $-2.888\pm0.001$) respectively. The slight underprediction of $\log_{10}(N_\mathrm{Ia})$ is likely due to the strong positive parameter correlation with $\alpha_\mathrm{IMF}$. This indicates that our neural network and sampling implementation is working as expected, since we can accurately predict the global galactic parameters from a data-set drawn directly from our model. The confidence intervals clearly shrink as we add more stars to the analysis, which is as expected, since the number of elemental data-points (here $n_\mathrm{el}n_\mathrm{stars}=8n_\mathrm{stars}$) becomes large compared to the number of free parameters ($2+4n_\mathrm{stars}$). For small $n_\mathrm{stars}$, we caution that our recovered galactic parameters may be strongly biased from the specific choice of stars used, but this bias shrinks when using many stars.

% \begin{figure*}
%     \centering
%     \includegraphics[width=0.9\textwidth]{TNGComparison.pdf}
%     \caption{\oliver{to remake}Inferred bounds on the global galactic parameters $\vec\Lambda$ from an IllustrisTNG galaxy \citep{2018MNRAS.475..648P}, computed for various sized data-sets using three inference routines. Beyond $n_\mathrm{stars}=100$ \oliver{check}, data is only given for the `Group' ADVI \oliver{check nomenclature} sampling technique, since this has the smallest computational cost. \oliver{what are we plotting? median and 1-sigma?} Unlike in Fig.\,\ref{fig: mock_comparison}, we only perform one analysis for each value of $n_\mathrm{stars}$, thus we note significant selection bias in the inferred parameters when using few stars. \oliver{check conclusions}The methods are clearly in agreement across the range of $n_\mathrm{stars}$, albeit with a slight overestimation by `Group ADVI' as $n_\mathrm{stars}\rightarrow1$. As $n_\mathrm{stars}$ becomes large, $\alpha_\mathrm{IMF}$ becomes very close to the true value of $-2.3$, but we report a minor ($\sim2\%$) discrepancy in $\log_{10}(N_\mathrm{Ia})$ from the true value of $-2.89$.}
%     \label{fig: TNG_comparison}
% \end{figure*}

%\oliver{add timing comparison here?}
% \begin{figure*}
%     \centering
%     \includegraphics[width=0.4\textwidth]{TNGComparisonTimes.pdf}
% \caption{\oliver{to remake}\oliver{redo caption} Sampling timescales for the parameter inferences shown in Fig.\,\ref{fig: mock_comparison} using the \textit{Chempy} mock data, showing the total run-time as a function of the number of stellar data-points, $n_\mathrm{stars}$. For the ADVI routines, this is the time to fit a multivariate Gaussian to the posterior such that the loss falls by less than $0.1\%$ in 10,000 fitting steps, whilst for HMC it is the total run-time to compute 8000 posterior chain samples \oliver{or 16,000?}. HMC is normally run on multiple cores; the 1-core dataset shows the equivalent sampling time if run single-threaded. Beyond $n_\mathrm{stars} = 200$ \oliver{or 100?}, the sampling times for Full Rank ADVI and HMC become very large and are not included. \oliver{Add in emcee sampling times?}}\label{fig: TNG_times}
% \end{figure*}


%% This command is needed to show the entire author+affilation list when
%% the collaboration and author truncation commands are used.  It has to
%% go at the end of the manuscript.
%\allauthors

%% Include this line if you are using the \added, \replaced, \deleted
%% commands to see a summary list of all changes at the end of the article.
%\listofchanges


